$k$-Neighbor Based Curriculum Sampling for Sequence Prediction

Multi-step ahead prediction in language models is challenging due to the discrepancy between training and test time processes. At test time, a sequence predictor is required to make predictions given past predictions as the input, instead of the past targets that are provided during training. This difference, known as exposure bias, can lead to the compounding of errors along a generated sequence at test time. To improve generalization in neural language models and address compounding errors, we propose \textit{Nearest-Neighbor Replacement Sampling} -- a curriculum learning-based method that gradually changes an initially deterministic teacher policy to a stochastic policy. A token at a given time-step is replaced with a sampled nearest neighbor of the past target with a truncated probability proportional to the cosine similarity between the original word and its top $k$ most similar words. This allows the learner to explore alternatives when the current policy provided by the teacher is sub-optimal or difficult to learn from. The proposed method is straightforward, online and requires little additional memory requirements. We report our findings on two language modelling benchmarks and find that the proposed method further improves performance when used in conjunction with scheduled sampling.

==> notes/training_details.tex <==
\iffalse In our experiments we use the aforementioned architecture used in ~\cite{sutskever2014sequence} as the basis for our experiments.\fi
\iffalse or unnecessarily complicated architectures which will let us easier identify whether performance gains or losses are due to the proposed technique.\fi


\iffalse
The LSTM consists of 2-hidden layers with a embedding dimension and hidden dimension size $|x|=|h|=200$. Xavier uniform initialization is used with $(\mu = 0, \sigma = 0.1)$ and gradients are clipped at $0.5$ threshold if exceeded at each update, with a batch size $|X_s|=30$.
\fi
\iffalse
Encoder and decoder weights are tied in the network which reduces the number of parameters and therefore can be considered a form of regularization. From an information theoretic point of view, ~\cite{shwartz2017opening} showed that the encoder performs input data compression with high mutual information between the input and encoder for the most epochs while the decoder has lower mutual information with the target. This is then reversed towards the end of training whereby the information in the network diffuses. We argue this what allows us to tie weights and still perform relatively well since most time is taken efficiently representing the input and less time spent on fitting the training labels, particularly relevant in NLM's since the input and output share the same space. 
\fi
\iffalse the learning rate decays over time starting at $10 \to 0$\fi
\iffalse
Encoder and decoder weights are tied in the network to reduce the number of parameters. 
\fi
